How to Test the Randomness from the Wireless Channel for Security?

We revisit the traditional framework of wireless secret key generation, where two parties leverage the wireless channel randomness to establish a secret key. The essence in the framework is to quantify channel randomness into bit sequences for key generation. Conducting randomness tests on such bit sequences has been a common practice to provide the confidence to validate whether they are random. Interestingly, despite different settings in the tests, existing studies interpret the results the same: passing tests means that the bit sequences are indeed random. In this paper, we investigate how to properly test the wireless channel randomness to ensure enough security strength and key generation efficiency. In particular, we define an adversary model that leverages the imperfect randomness of the wireless channel to search the generated key, and create a guideline to set up randomness testing and privacy amplification to eliminate security loss and achieve efficient key generation rate. We use theoretical analysis and comprehensive experiments to reveal that common practice misuses randomness testing and privacy amplification: (i) no security insurance of key strength, (ii) low efficiency of key generation rate. After revision by our guideline, security loss can be eliminated and key generation rate can be increased significantly.

==> Makefile <==
# Makefile for tex files: tex->dvi->ps->pdf
# This makefile automatically searches and compiles each tex file respectively.

# Colloct all tex sources
TEXSRCS := $(wildcard *.tex)
# TEXSRCS := [YOUR TARGET].tex

# _region_.tex is generated by AUCTEX
# Therefore we ignore this tex file

IGNORE = _region_.tex
TEXSRCSORG := $(TEXSRCS)
TEXSRCS := $(TEXSRCS:$(IGNORE)=)

IGNORE = AddrDiff.tex
TEXSRCSORG := $(TEXSRCS)
TEXSRCS := $(TEXSRCS:$(IGNORE)=)

# Get all pdf, dvi and ps files
TARGETS := $(TEXSRCS:.tex=.pdf)
DVIFILES := $(TEXSRCS:.tex=.dvi)
PSFILES := $(TEXSRCS:.tex=.ps)

# Temp files
TMPTEXFILE = TMPTEXFILE.out
TMPBIBFILE = TMPBIBFILE.out

# Define commands and args
CMD_LATEX=latex
CMD_BIBTEX=bibtex
CMD_DVIPS=dvips
CMD_PSPDF=ps2pdf13

LATEX_ARGS=-src-specials -interaction=nonstopmode #-file-line-error-style 
DVIPS_ARGS=-q -t letter
ERR_INFO='Error | Undefined | Missing |^l\.|! Double | not found'

############################################
# Start Objectives

all: cleanall $(TARGETS) clean
dvi: cleanall $(DVIFILES) deltemp_nodvi
noclean: $(TARGETS)

$(DVIFILES): %.dvi : %.tex
	@echo '$----------------------------';\
	echo "  $< -> $@...";\
	$(CMD_LATEX) $(LATEX_ARGS) $< >$(TMPTEXFILE);\
	grep -E $(ERR_INFO) $(TMPTEXFILE);\
	$(CMD_BIBTEX) $(basename $<) >$(TMPBIBFILE);\
	$(CMD_LATEX) $(LATEX_ARGS) $(basename $<) > $(TMPTEXFILE);\
	$(CMD_LATEX) $(LATEX_ARGS) $(basename $<) > $(TMPTEXFILE);

$(PSFILES): %.ps : %.dvi
	@echo "  $< -> $@...";\
	$(CMD_DVIPS) $(DVIPS_ARGS) -o $@ $<;

$(TARGETS): %.pdf : %.ps
	@echo "  $< -> $@...";\
	$(CMD_PSPDF) $<;

.PONY: all dvi noclean clean cleanall deltemp_nodvi

clean: $(TEXSRCSORG)
	@rm -f $(TEXSRCSORG:.tex=.dvi) $(TEXSRCSORG:.tex=.ps) $(TEXSRCSORG:.tex=.toc) $(TEXSRCSORG:.tex=.log) $(TEXSRCSORG:.tex=.blg) $(TEXSRCSORG:.tex=.bbl) $(TEXSRCSORG:.tex=.aux) $(TEXSRCSORG:.tex=.out) $(TMPTEXFILE) $(TMPBIBFILE) 

deltemp_nodvi: $(TEXSRCSORG)
	@rm -f $(TEXSRCSORG:.tex=.ps) $(TEXSRCSORG:.tex=.toc) $(TEXSRCSORG:.tex=.log) $(TEXSRCSORG:.tex=.blg) $(TEXSRCSORG:.tex=.bbl) $(TEXSRCSORG:.tex=.aux) $(TEXSRCSORG:.tex=.out) $(TMPTEXFILE) $(TMPBIBFILE) 

cleanall: $(TEXSRCSORG)
	@rm -rf _region_.prv;rm -f $(TEXSRCSORG:.tex=.pdf) $(TEXSRCSORG:.tex=.dvi) $(TEXSRCSORG:.tex=.ps) $(TEXSRCSORG:.tex=.toc) $(TEXSRCSORG:.tex=.log) $(TEXSRCSORG:.tex=.blg) $(TEXSRCSORG:.tex=.bbl) $(TEXSRCSORG:.tex=.aux) $(TEXSRCSORG:.tex=.out) $(TMPTEXFILE) $(TMPBIBFILE) _region_.* prv_*.log;

